Reaction-diffusion spatial modeling of COVID-19: Greece and Andalusia as case examples

We examine the spatial modeling of the outbreak of COVID-19 in two regions: the autonomous community of Andalusia in Spain and the mainland of Greece. We start with a 0D compartmental epidemiological model consisting of Susceptible, Exposed, Asymptomatic, (symptomatically) Infected, Hospitalized, Recovered, and deceased populations. We emphasize the importance of the viral latent period and the key role of an asymptomatic population. We optimize model parameters for both regions by comparing predictions to the cumulative number of infected and total number of deaths via minimizing the $\ell^2$ norm of the difference between predictions and observed data. We consider the sensitivity of model predictions on reasonable variations of model parameters and initial conditions, addressing issues of parameter identifiability. We model both pre-quarantine and post-quarantine evolution of the epidemic by a time-dependent change of the viral transmission rates that arises in response to containment measures. Subsequently, a spatially distributed version of the 0D model in the form of reaction-diffusion equations is developed. We consider that, after an initial localized seeding of the infection, its spread is governed by the diffusion (and 0D model "reactions") of the asymptomatic and symptomatically infected populations, which decrease with the imposed restrictive measures. We inserted the maps of the two regions, and we imported population-density data into COMSOL, which was subsequently used to solve numerically the model PDEs. Upon discussing how to adapt the 0D model to this spatial setting, we show that these models bear significant potential towards capturing both the well-mixed, 0D description and the spatial expansion of the pandemic in the two regions. Veins of potential refinement of the model assumptions towards future work are also explored.

==> Tables/table_parameters.tex <==
\begin{tabular}{cccccc} 
\hline \hline 
& & Greece & Greece & Andalusia & Andalusia\\ 
& & $(t_q=13)$ & $(t_q=23)$ & $(t_q=3)$ & $(t_q=16)$\\ 
\hline 
Population & $N$ & \multicolumn{2}{c}{10,768,477} & \multicolumn{2}{c}{8,414,240} \\Initial populations & ($I_0, H_0, D_0$) & \multicolumn{2}{c}{(117,0,1)} & \multicolumn{2}{c}{(297, 134, 6)} \\Non COVID-19 death rate [per day] & $\mu$ & \multicolumn{2}{c}{$8.49 \times 10^{-6}$} & \multicolumn{2}{c}{$5.79 \times 10^{-7}$} \\Transmission rate, $S \rightarrow I$ [per day] & $\beta_{IS} \ ^{\star}$ & 0.31 (0.29--0.33) & 0.24 (0.23--0.25) & 0.35 (0.28--0.41) & 0.32 (0.29--0.35) \\ 
Transmission rate, $S \rightarrow A$ [per day] & $\beta_{AS} \ ^{\star}$ & 0.21 (0.19--0.22) & 0.18 (0.17--0.19) & 0.55 (0.50--0.60) & 0.28 (0.26--0.30) \\ 
Lockdown effect, $S \rightarrow I$ & $\eta_{IS,1}$ & 0.52 (0.49--0.54) & 0.48 (0.46--0.50) & 0.28 (0.24--0.35) & 0.39 (0.36--0.42) \\ 
Lockdown effect, $S \rightarrow A$ & $\eta_{AS,1}$ & 0.52 (0.49--0.54) & 0.48 (0.46--0.50) & 0.48 (0.43--0.56) & 0.38 (0.35--0.41) \\ 
Latency period, $A \rightarrow I$ [days] & $1/\sigma_A$ & 2.82 (2.76--2.89) & 2.89 (2.81--2.97) & 4.52 (4.36--4.69) & 2.97 (2.87--3.05) \\ 
Incubation period, $E \rightarrow I$ [days] & $1/\sigma_I$ & 4.38 (4.14--4.68) & 3.72 (3.55--4.00) & 3.15 (2.98--3.33) & 3.77 (3.54--4.14) \\ 
Infectivity period [days] & $1/M$ & 6.30 (6.24--6.37) & 6.13 (6.07--6.19) & 6.06 (5.98--6.12) & 5.97 (5.89--6.04) \\ 
Recovery period (asymptomatics), $A \rightarrow AR$ [days] & $1/M_{AR}$ & 6.95 (6.89--7.02) & 6.87 (6.80--6.96) & 6.15 (6.08--6.21) & 6.85 (6.75--6.94) \\ 
Recovery period (hospitalized), $H \rightarrow R$ [days] & $1/\chi$ & 6.36 (6.31--6.42) & 6.20 (6.16--6.26) & 8.39 (8.23--8.54) & 6.74 (6.60--6.85) \\ 
Period from hospitalized to deceased, $H \rightarrow D$ [days] & $1/\psi$ & 8.87 (8.75--9.00) & 8.76 (8.62--8.92) & 9.38 (9.22--9.57) & 8.33 (8.17--8.53) \\ 
Conversion fraction ($I \overset{\gamma}{\longrightarrow} H$, $I \overset{1-\gamma}{\longrightarrow} R$) & $\gamma$ & 0.44 (0.43--0.44) & 0.44 (0.43--0.45) & 0.58 (0.57--0.59) & 0.55 (0.54--0.57) \\ 
Conversion fraction ($H \overset{\omega}{\longrightarrow} D$, $H \overset{1-\omega}{\longrightarrow} R$) & $\omega$ & 0.22 (0.21--0.22) & 0.21 (0.21--0.22) & 0.25 (0.24--0.26) & 0.25 (0.25--0.26) \\ 
Initial population fraction, exposed & $\epsilon_E = E_0/I_0$ & 2.65 (2.39--3.01) & 2.71 (2.51--3.04) & 2.90 (2.39--3.27) & 2.69 (2.42--3.14) \\ 
Initial population fraction, asymptomatic & $\epsilon_A = A_0/I_0$ & 2.84 (2.44--3.16) & 2.87 (2.59--3.18) & 3.33 (2.92--3.77) & 2.93 (2.59--3.34) \\ 
Diffusivity, $S$ [km$^2$/day] & $D_{S,1}$ & 10 & 10 & --- & 10 \\Diffusivity, $E$ or $A$ [km$^2$/day] & $D_{E,1}$ or $D_{A,1}$ & 100 & 100 & --- & 100 \\\hline \hline 
\end{tabular} 

